Dynamic Relation Repairing for Knowledge Enhancement

Dynamic relation repair aims to efficiently validate and repair the instances for knowledge graph enhancement (KGE), where KGE captures missing relations from unstructured data and leads to noisy facts to the knowledge graph. With the prosperity of unstructured data, an online approach is asked to clean the new RDF tuples before adding them to the knowledge base. To clean the noisy RDF tuples, graph constraint processing is a common but intractable approach. Plus, when adding new tuples to the knowledge graph, new graph patterns would be created, whereas the explicit discovery of graph constraints is also intractable. Therefore, although the dynamic relation repair has an unfortunate hardness, it is a necessary approach for enhancing knowledge graphs effectively under the fast-growing unstructured data. Motivated by this, we establish a dynamic repairing and enhancing structure to analyze its hardness on basic operations. To ensure dynamic repair and validation, we introduce implicit graph constraints, approximate graph matching, and linkage prediction based on localized graph patterns. To validate and repair the RDF tuples efficiently, we further study the cold start problems for graph constraint processing. Experimental results on real datasets demonstrate that our proposed approach can capture and repair instances with wrong relation labels dynamically and effectively.

==> ACMTP-Relation repairing/pic/errorrate/errorRate-precision.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(7200.00,5040.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(814,704){\makebox(0,0)[r]{\strut{}$0$}}%
      \put(814,1112){\makebox(0,0)[r]{\strut{}$0.1$}}%
      \put(814,1521){\makebox(0,0)[r]{\strut{}$0.2$}}%
      \put(814,1929){\makebox(0,0)[r]{\strut{}$0.3$}}%
      \put(814,2337){\makebox(0,0)[r]{\strut{}$0.4$}}%
      \put(814,2746){\makebox(0,0)[r]{\strut{}$0.5$}}%
      \put(814,3154){\makebox(0,0)[r]{\strut{}$0.6$}}%
      \put(814,3562){\makebox(0,0)[r]{\strut{}$0.7$}}%
      \put(814,3971){\makebox(0,0)[r]{\strut{}$0.8$}}%
      \put(814,4379){\makebox(0,0)[r]{\strut{}$0.9$}}%
      \put(946,484){\makebox(0,0){\strut{}$2$}}%
      \put(1597,484){\makebox(0,0){\strut{}$4$}}%
      \put(2248,484){\makebox(0,0){\strut{}$6$}}%
      \put(2898,484){\makebox(0,0){\strut{}$8$}}%
      \put(3549,484){\makebox(0,0){\strut{}$10$}}%
      \put(4200,484){\makebox(0,0){\strut{}$12$}}%
      \put(4851,484){\makebox(0,0){\strut{}$14$}}%
      \put(5501,484){\makebox(0,0){\strut{}$16$}}%
      \put(6152,484){\makebox(0,0){\strut{}$18$}}%
      \put(6803,484){\makebox(0,0){\strut{}$20$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(198,2541){\rotatebox{-270}{\makebox(0,0){\strut{}Precision}}}%
      \put(3874,154){\makebox(0,0){\strut{}Error rate (%)}}%
      \put(3874,4709){\makebox(0,0){\strut{}(a)}}%
      \csname LTb\endcsname%%
      \put(5816,2761){\makebox(0,0)[r]{\strut{}JointE+S5}}%
      \csname LTb\endcsname%%
      \put(5816,2541){\makebox(0,0)[r]{\strut{}JointE+S10}}%
      \csname LTb\endcsname%%
      \put(5816,2321){\makebox(0,0)[r]{\strut{}JointE+S20}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{errorRate-precision}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> pic/errorrate/errorRate-precision.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(7200.00,5040.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(814,704){\makebox(0,0)[r]{\strut{}$0$}}%
      \put(814,1112){\makebox(0,0)[r]{\strut{}$0.1$}}%
      \put(814,1521){\makebox(0,0)[r]{\strut{}$0.2$}}%
      \put(814,1929){\makebox(0,0)[r]{\strut{}$0.3$}}%
      \put(814,2337){\makebox(0,0)[r]{\strut{}$0.4$}}%
      \put(814,2746){\makebox(0,0)[r]{\strut{}$0.5$}}%
      \put(814,3154){\makebox(0,0)[r]{\strut{}$0.6$}}%
      \put(814,3562){\makebox(0,0)[r]{\strut{}$0.7$}}%
      \put(814,3971){\makebox(0,0)[r]{\strut{}$0.8$}}%
      \put(814,4379){\makebox(0,0)[r]{\strut{}$0.9$}}%
      \put(946,484){\makebox(0,0){\strut{}$2$}}%
      \put(1597,484){\makebox(0,0){\strut{}$4$}}%
      \put(2248,484){\makebox(0,0){\strut{}$6$}}%
      \put(2898,484){\makebox(0,0){\strut{}$8$}}%
      \put(3549,484){\makebox(0,0){\strut{}$10$}}%
      \put(4200,484){\makebox(0,0){\strut{}$12$}}%
      \put(4851,484){\makebox(0,0){\strut{}$14$}}%
      \put(5501,484){\makebox(0,0){\strut{}$16$}}%
      \put(6152,484){\makebox(0,0){\strut{}$18$}}%
      \put(6803,484){\makebox(0,0){\strut{}$20$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(198,2541){\rotatebox{-270}{\makebox(0,0){\strut{}Precision}}}%
      \put(3874,154){\makebox(0,0){\strut{}Error rate (%)}}%
      \put(3874,4709){\makebox(0,0){\strut{}(a)}}%
      \csname LTb\endcsname%%
      \put(5816,2761){\makebox(0,0)[r]{\strut{}JointE+S5}}%
      \csname LTb\endcsname%%
      \put(5816,2541){\makebox(0,0)[r]{\strut{}JointE+S10}}%
      \csname LTb\endcsname%%
      \put(5816,2321){\makebox(0,0)[r]{\strut{}JointE+S20}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{errorRate-precision}}%
    \gplfronttext
  \end{picture}%
\endgroup

